Planning profitable tours for field sales forces: A unified view on sales analytics and mathematical optimization

Field sales forces play an important role in direct marketing, especially for companies offering complex products, services, or solutions in the business-to-business context. A key task of sales representatives in operational planning is to select the most promising customers to visit within the next days. On an operative horizon, a key task for sales representatives is to select the most promising customers to visit within the next days. A strongly varying set of scoring methods predicting or approximating the expected response exists for this customer selection phase. However, in the case of field sales forces, the final customer selection is strongly interrelated to the tour planning decisions. To this end, we formalize variants of the profitable sales representatives tour problem as a multi-period team orienteering problem, thereby providing a unified view on the customer scoring and the tour planning phase. In an extensive computational study on real-world instances from the retail industry, we systematically examine the impact of the aggregation level and the content of information provided by a scoring method and the sensitivity of the proposed models concerning prediction errors. We show that the selection of a customer scoring and tour planning variant depends on the available data. Furthermore, we work out where to put effort in the data acquisition and scoring phase to get better operational tours.

==> 04_solution_approach.tex <==
\section{Adaptive large neighborhood search with multi-start}

\comment{Umgestellt und gekürzt - klappt das?}

For solving large-scale instances of the MP-OP, we apply an adaptive large neighborhood search (ALNS) based on the concepts introduced by \cite{Ropke2006} together with a multi-start phase for quickly identifying promising starting solutions. 
\revised{
The main purpose of this algorithm is to adapt and combine heuristic promising solution concepts from literature that can be applied to all modeling variants introduced above. 
This gives us reason to believe that the insights obtained in our study can be transferred to similar problems and solution approaches.
}

\revised{
Similar to the solution concepts discussed in Section \ref{sec:orienteering_literature}, we combine neighborhoods that focus on improving the sum of scores of the selected customers with others that seek to improve the efficiency of the obtained tours.
These are implemented in form of adapted removal and insertion strategies in the ALNS, which are briefly discussed below. 
We then introduce the multi-start strategy and the reheating scheme that guides the search.}

\subsection{Removal strategies}

Removal strategies remove a given percentage of customer nodes from a solution following relatively simple heuristic rules.
\revised{Based on a series of preliminary tests,} the number of customers selected for removal is in $[\max\{0.1 |\mathcal{N}^C|, 10\}, \min\{0.3 |\mathcal{N}^C|, 100\}]$.
In our implementation, unvisited customers have to be explicitly removed from a solution as well.
Otherwise, they cannot be re-inserted in the subsequent repair step.
Unless otherwise noted, the unvisited customers to be removed are neighbors of those removed from the tours.
The purpose of this is to limit the size of the neighborhood in each iteration and to reduce the computational effort due to evaluating customers that are not likely to be re-inserted. 
Our ALNS uses six different removal strategies:
\begin{description}
\item[RND-NN] removes visited customers at random.
\item[SEQU-NN] removes sequences of customers from the tours.
\item[SCORE-DELTA] removes the planned customers with the lowest scores as well as the unvisited customers with the highest scores from a solution.
\item[SKEL-TOUR] randomly selects one tour and removes all customer visits within this tour in segments of a fixed length, leaving one customer in between subsequent segments. This results in a ``skeleton'' tour with the same basic structure as the initial one.
\item[WORST-DETOUR] removes customers associated with high travel times.
\item[WORST-ANGLE] selects customers that come with sharp angles in a tour as well as the preceding and succeeding customers.
\end{description}


\subsection{Insertion strategies}

Insertion strategies iteratively select one of the removed customers and try to reinsert it into a tour.
Strategies vary in the order of insertions. 
If there are mandatory customers, i.e., $\mathcal{N}^{M} \neq \emptyset$, they are inserted first; if the insertion is not feasible, the repair phase ends.
The insertion strategies are:
\begin{description}
\item[RND] inserts customers in random order.
\item[MAX-SCORE] inserts the remaining customer with the highest score first.
\item[SCORE-RATIO] calculates the ratios of the customers' scores with the associated detours for the best insertion positions and inserts the one with the best ratio first.
\item[SCORE-RATIO2] similarly computes the score ration but uses the squared score values.
\item[GREEDY] inserts customers in increasing order of the necessary detour, irrespective of their score.
\end{description}
All strategies (except RND) are slightly randomized so that in each iteration, an arbitrary customer is selected for insertion with a probability of $0.05$ to encourage diversification.

The selected customers are inserted at the position that is currently associated with the lowest detour with respect to the emerging tours.
If no position remains that is feasible with respect to the working time constraint, the customer is left unvisited in the solution.

\subsection{Seeds and multi-start}

Initial solutions are created in a multi-start approach.
First, we select seed nodes for each day from the set of customers using a k-means++ variant, which means that the likelihood of a customer to be selected as seed increases with its distance towards other seeds and the home location \citep{Arthur2006}. 
If there are mandatory customers, the seeds are chosen from the set $\mathcal{N}^{M}$.
Each seed initializes one tour.
Then, one of the insertion strategies is applied to build tours for each day.
This is repeated 10 times using different insertion strategies.
The best solution obtained this way is used as a starting solution for the ALNS. 


\subsection{Acceptance and stopping criterion}

During the search, improving solutions are always accepted.
Similar to \cite{Vidal2015}, we use travel distance as a tiebreaker for solutions with similar scores.
This way, the ALNS prefers solutions visiting the same customers at a lower cost.
We furthermore apply a reheating scheme related to simulated annealing (SA) to guide the search.
This scheme accepts solutions that come with a decrease in solution quality with a probability that increases with the number of iterations since the best solution was last improved.
Decreases in quality are only accepted if the search has likely resulted in a local minimum that cannot be left otherwise.
The search stops when no improvements over the current best solution have been found in 300 iterations.

==> todo_notes.tex <==
\def\includetodos{active}		%comments active or inactive 
\def\highlightchanges{active}

\usepackage[colorinlistoftodos]{todonotes} 

\ifthenelse{\equal{\includetodos}{active}}{
%% Comments
  \newcommand{\TODO}[1]{\todo[inline, size=\small]{TODO: #1}}                                   %% ToDo Tasks
  \newcommand{\comment}[1]{\todo[inline, size=\small, color=red!40]{#1}}
  \newcommand{\formulation}[1]{\todo[inline, size=\small, color=purple!40]{check formulation: #1}}
}{}

\ifthenelse{\equal{\includetodos}{inactive}}{
  \newcommand{\comment}[1]{}                 %% Comment
  \newcommand{\TODO}[1]{}                    %% ToDo Tasks
  \newcommand{\formulation}[1]{#1}
}{}


\usepackage[normalem]{ulem}
\usepackage{xcolor}
\ifthenelse{\equal{\highlightchanges}{active}}{
	\newcommand{\revised}[1]{\textcolor{ForestGreen}{#1}}
	\newcommand{\deleted}[1]{\textcolor{BurntOrange}{\sout{#1}}}
}{
	\newcommand{\revised}[1]{#1}
	\newcommand{\deleted}[1]{}	% do not show if inactive
}

